The Exotic Zoo of Millisecond Pulsars in Globular Clusters: a multi-wavelength study

This thesis work is focused on the study of millisecond pulsars in globular cluster by using multi-wavelength observations obtained with radio and optical telescopes. Radio observations have been used to search for and timing the pulsars. While classical search routines are based on the analysis of single and long time sequence of data, we present here an alternative method. This method exploits the large amount of available archival radio data to search for very faint pulsars by stacking all the daily power spectra. This method led to the discovery of three new pulsars in the stellar system Terzan 5. Optical observations have been exploited to search for millisecond pulsar optical counterparts, whose emission is totally dominated by the companion stars. Six new companion stars have been discovered, thus increasing by ~40% the total number of companions identified in globular clusters. In particular, four companions turned out to be He white dwarfs, as expected from the canonical formation scenario. One companion turned out to be a very faint and non-degenerate object, showing a strong variability which is likely the result of a strong heating of the stellar side exposed to the pulsar injected flux. Finally, one companion is a main-sequence star which shows a strong H{\alpha} emission likely due to a low-level accretion probably from a residual disk. This system can be located in an early evolutive stage, immediately preceding the reactivation of an already re-accelerated pulsar. Furthermore, we identified the companion star to a transient low-mass X-ray binary. Conclusion are drawn in the final chapter, where the evolution of millisecond pulsars is discussed and possible future developments are suggested.

==> frontmatter/abstract.tex <==
%
% File: abstract.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the text for thesis abstract
%
% UoB guidelines:
%
% Each copy must include an abstract or summary of the dissertation in not
% more than 300 words, on one side of A4, which should be single-spaced in a
% font size in the range 10 to 12. If the dissertation is in a language other
% than English, an abstract in that language and an abstract in English must
% be included.

\chapter*{Abstract}
\begin{SingleSpace}
\initial{H}ere goes the abstract
\end{SingleSpace}
\clearpage

==> frontmatter/declaration.tex <==
%
% File: declaration.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the declaration page
%
% UoB guidelines:
%
% Author's declaration
%
% I declare that the work in this dissertation was carried out in accordance
% with the requirements of the University's Regulations and Code of Practice
% for Research Degree Programmes and that it has not been submitted for any
% other academic award. Except where indicated by specific reference in the
% text, the work is the candidate's own work. Work done in collaboration with,
% or with the assistance of, others, is indicated as such. Any views expressed
% in the dissertation are those of the author.
%
% SIGNED: .............................................................
% DATE:..........................
%
\chapter*{Author's declaration}
\begin{SingleSpace}
\begin{quote}
\initial{I} declare that the work in this dissertation was carried out in accordance with the requirements of  the University's Regulations and Code of Practice for Research Degree Programmes and that it  has not been submitted for any other academic award. Except where indicated by specific  reference in the text, the work is the candidate's own work. Work done in collaboration with, or with the assistance of, others, is indicated as such. Any views expressed in the dissertation are those of the author.

\vspace{1.5cm}
\noindent
\hspace{-0.75cm}\textsc{SIGNED: .................................................... DATE: ..........................................}
\end{quote}
\end{SingleSpace}
\clearpage

==> frontmatter/title.tex <==
%
% File: Title.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the title page
%
% UoB guidelines:
% 
% At the top of the title page, within the margins, the dissertation should give the title and, if 
% necessary, sub-title and volume number. If the dissertation is in a language other than English, the 
% title must be given in that language and in English. The full name of the author should be in the 
% centre of the page. At the bottom centre should be the words ?A dissertation submitted to the 
% University of Bristol in accordance with the requirements for award of the degree of ? in the 
% Faculty of ...?, with the name of the school and month and year of submission. The word count of 
% the dissertation (text only) should be entered at the bottom right-hand side of the page.
%
%
\begin{titlingpage}
\begin{SingleSpace}
\calccentering{\unitlength} 
\begin{adjustwidth*}{\unitlength}{-\unitlength}
\vspace*{13mm}
\begin{center}
\rule[0.5ex]{\linewidth}{2pt}\vspace*{-\baselineskip}\vspace*{3.2pt}
\rule[0.5ex]{\linewidth}{1pt}\\[\baselineskip]
{\HUGE University of Bologna }\\[4mm]
{\Large \textit{Science School}}\\
\rule[0.5ex]{\linewidth}{1pt}\vspace*{-\baselineskip}\vspace{3.2pt}
\rule[0.5ex]{\linewidth}{2pt}\\
\vspace{6.5mm}
{\large By}\\
\vspace{6.5mm}
{\large\textsc{Mario Cadelano}}\\
\vspace{11mm}
\includegraphics[scale=0.3]{logos/alma.jpg}\\
\vspace{6mm}
{\large Department of Physics and Astronomy\\
\textsc{University of Bologna}}\\
\vspace{11mm}
\begin{minipage}{10cm}
The exotic zoo of millisecond pulsar in globular clusters: a multi-wavelength study\end{minipage}\\
\vspace{9mm}
{\large\textsc{June 2017}}
\vspace{12mm}
\end{center}
\begin{flushright}
{\small May the force be with me}
\end{flushright}
\end{adjustwidth*}
\end{SingleSpace}
\end{titlingpage}
